Federated Alternate Training (FAT): Leveraging Unannotated Data Silos in Federated Segmentation for Medical Imaging

Federated Learning (FL) aims to train a machine learning (ML) model in a distributed fashion to strengthen data privacy with limited data migration costs. It is a distributed learning framework naturally suitable for privacy-sensitive medical imaging datasets. However, most current FL-based medical imaging works assume silos have ground truth labels for training. In practice, label acquisition in the medical field is challenging as it often requires extensive labor and time costs. To address this challenge and leverage the unannotated data silos to improve modeling, we propose an alternate training-based framework, Federated Alternate Training (FAT), that alters training between annotated data silos and unannotated data silos. Annotated data silos exploit annotations to learn a reasonable global segmentation model. Meanwhile, unannotated data silos use the global segmentation model as a target model to generate pseudo labels for self-supervised learning. We evaluate the performance of the proposed framework on two naturally partitioned Federated datasets, KiTS19 and FeTS2021, and show its promising performance.

==> sec/Proposed_Method.tex <==
\section{Proposed methods}
\label{sec:proposedmethod}
Federated Optimization focuses on a distributed optimization task where K nodes collaborate with each other to learn a global model with parameters $\theta$ as shown below,
\begin{equation}
    \min_{\theta} G(\mathcal{L}_{1}(\theta; X_{1}, Y_{1}), ..., \mathcal{L}_{K}(\theta; X_{K}, Y_{K})),
\end{equation}
where $\mathcal{L}(\theta_{i}; X_{i}, Y_{i})$ represents node i's local loss function, $X_{i}$ denotes the training data and $Y_{i}$ represents the labels/notations at node $i$. $G(.)$ function aggregates the local objectives, for example,  $\sum_{k=1}^{K} \frac{N_{k}}{N} \cdot \mathcal{L}_k(\theta)$ is performed in Federated Averaging algorithm \cite{mcmahan2017communication}.
\subsection{Problem Formulation}
In a typical federated averaging setting, each node consists of annotated data ($X_{i}$, $Y_{i}$). However, it is very unlikely that all nodes have labels available. In such a setting, the optimization problem becomes, 
% our goal is to solve the following optimization problem,
\begin{equation}
\begin{split}
    \min_{\theta} G(\mathcal{L}_{1}(\theta; X_{1}, Y_{1}),..., \mathcal{L}_{S}(\theta; X_{S}, Y_{S}), \\ \mathcal{L}_{S+1}(\theta; X_{S+1}),..., \mathcal{L}_{K}(\theta; X_{K})),
    \end{split}
\end{equation}
where $S$ signifies the number of nodes that have annotated data. Hence, the objective is to learn a global model such that learning from the unsupervised nodes $\{S+1, .., K\}$ nodes along with supervised nodes increases the global model performance as compared to the global model learned from all the supervised nodes $\{1,.., S\}$ alone. 

% Hence, the goal is to learn a global model where some nodes have data with annotations $(X, Y)$ available for training and some nodes only have unannotated data $(X)$ available for training. Therefore, the task breaks down to performing learning at the unsupervised nodes $\{S+1, .., K\}$ such that the performance of the global model learned from all the nodes $\{1,..,S,S+1,.., K\}$ is better than the model obtained only from the supervised nodes $\{1, .., S\}$ federated learning.

\begin{figure*}[htb]

\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=17cm]{Figures/system.png}}
%  \vspace{2.0cm}
  % \centerline{System Model Diagram}\medskip
\end{minipage}

\caption{The proposed Federated Alternate Training (FAT) framework where we alternate training between Annotated Data Silos and Unannotated Data Silos. The Annotated Data Silos follow a supervised training module where they have ground truth labels available. The Unannotated Data Silos follow an unsupervised training module where the target model generates pseudo labels, y, for the model to perform training and learns from the online model via exponential moving average (ema).}
\label{fig:sysmodel}
\end{figure*}
\subsection{Pretraining}
Pretrained models have gained popularity in computer vision (CV) and natural language processing (NLP) tasks because of their potential to enhance accuracy, generalizability and robustness \cite{devlin2018bert, hendrycks2019using}. These off-the-shelf models have also shown promising capabilities to bridge the performance gap between centralized and federated learning for CV \cite{chen2022pre}, and NLP tasks \cite{tian2022fedbert}. For the given problem of semisupervised learning in medical regimes where nodes may have limited or no annotated data, we initialize our models from the models pretrained on other medical source datasets and found them beneficial to obtain significant gains over the random model initializations. 

\subsection{Mixup Logic based Data Augmentations}
Data augmentations have shown huge benefits, especially in semi-supervised and unsupervised learning regimes. However, the task to determine the right choice of data augmentations, that bring data points near the decision boundary where data points are most likely to be misclassified, requires a lot of training data. In data-limited regimes such as ours, this approach may not always work due to limited data and pre-determined augmentations may not add perturbations to the adversarial directions for all the datasets. Therefore, we exploit mixup logic that has been well explored for the classification and segmentation task. Mixup logic adds pixel-level perturbations to the image and maintains consistency between the perturbed input's output and the perturbed outputs of the original input images. For example, for the two randomly selected input images $x_1$ and $x_2$, we obtain original data points input and perturbed input $x^{'}$ in the following way,
\begin{equation}
\begin{split}
    % x &= concat(x_1, x_2) \\
    x^{'} &= \lambda x_1 + (1 - \lambda) x_2
    \end{split}
\end{equation}
where $\lambda \in (0, 1)$ and is a hyperparameter.
\subsection{Bootstrapping}
Since we have unsupervised nodes, silos with unannotated data, in our network, we perform unsupervised learning at these silos.
During unsupervised training at these silos, our goal is to learn from the global model without completely forgetting what we learned from the supervised silos. Therefore, we bootstrap the learnt labels. That is, instead of maintaining one neural architecture, as is used in the previous work \cite{yang2021federated}, we maintain two neural architectures referred to as online with parameters $\xi$ and target with parameters $\theta$ models. Unsupervised silos initialize both of these models with the global model at each round. The goal of online model is to output the prediction probabilities $g_{mix}$ of each class for the perturbed input $x^{'}$ and the target model outputs the prediction probabilities $g$ of each class of the unperturbed images $x_1$ and $x_2$. The softmax outputs of the target models are perturbed via mixup logic as follows,
\begin{equation}
\begin{split}
    % g_1&, g_2 = unconcat(g) \\
    p^{'} &= \lambda p_1 + (1 - \lambda) p_2
    \end{split}
\end{equation}
The pseudo label $y$ is obtained by applying argmax operation on the perturbed output $p^{'}$. Hence, the target model provides the target labels for the online model to perform unsupervised learning. After each training step of the online model, the target model is updated by the following exponential moving average,
\begin{equation}
\theta = \tau \theta + (1 - \tau) \xi,
\end{equation}
where $\tau \in (0, 1)$ is a decay rate of the target model. To train the online model, we use Dice loss and Cross Entropy loss between the pseudo label $y$ and $p_{mix}$ at the unsupervised silo. At the supervised silos, since we do not need pseudo labels, we train only one model with parameters $\theta$, and use Dice loss and Cross Entropy loss between the ground truth label $y$ and the model predicted probabilities $g$ for learning as shown in Fig \ref{fig:sysmodel}.
% Explain why data augmentations need a lot of data to determine the right choice as is the case with GANs and how Mixup logic can be a sophisticated solution. Write the mixup equations.
\subsection{Alternate Training}
In addition to exploiting the supervised pretraining at other datasets, we also alternate training between the supervised and unsupervised silos for the given dataset in our network. In alternate training, we first train our model at the supervised silos alone for a few communication rounds. Next, we send the global model aggregated from supervised silos to the unsupervised silos alone, where they use this model as a target model to bootstrap the model-generated labels. We keep alternating the training between supervised and unsupervised silos until the global model is converged. We show from ablation studies that alternate training boosts performance by enhancing the quality of pseudo labels generated at the unsupervised silos.
% \subsection{Model predictions upon model receiving and Pseudo Labeling}
% Emphasize why model predictions can be better
% \subsection{Forgetting problem and Bootstrapping}
% EMA
\subsection{Model Aggregation}
For the model aggregation, we found the federated averaging algorithm objective function, i.e, $\sum_{k=1}^{K} \frac{N_{k}}{N} \cdot \mathcal{L}_k(\theta)$ with alternate training to work better than the weighted averaging objective, $\sum_{k=1}^{S} \frac{N_{k}}{N} \cdot \mathcal{L}_k(\theta) + \eta_{t} \sum_{k=S+1}^{K}  \frac{N_{k}}{N} \cdot \mathcal{L}_k(\theta)$ with/without alternate training. The weighted averaging is inspired by the centralized semi-supervised works where the weight $\eta_{t}$ increases by increasing $t$, where $t$ denotes the communication round number. We apply the Gaussian ramp-up curve $ e^{[-5(1-T)^2]}$, where T goes from 0 to 1 linearly to perform an ablation study. Note that since we perform alternate training therefore, our global objective alternates between $\sum_{k=1}^{S} \frac{N_{k}}{N} \cdot \mathcal{L}_k(\theta)$ and $\sum_{k=S+1}^{K} \frac{N_{k}}{N} \cdot \mathcal{L}_k(\theta)$.

% $G(.)$ function aggregates the local objectives, for example,  $\sum_{k=1}^{K} \frac{N_{k}}{N} \cdot \mathcal{L}_k(\theta)$ is performed in Federated Averaging algorithm
% Explain weight aggregation with and without weights.

\begin{algorithm}[htb]
    \caption{FAT Algorithm. }
    \begin{small}
        \begin{algorithmic}[1]
            \STATE \textbf{Initialization:} initialize ${\theta}_0$; $s$ represents the supervised client index where $k \in \{1,2,...,S\} $ and $u$ represents the unsupervised client index where $u \in \{S+1,S+2,...,K\} $  ; $E$ is the number of local epochs for each client; $T$ is the number of rounds, $A$ number of required rounds alternating between supervised and unsupervised clients, $DICE$ is the soft Dice loss function, $CE$ is the cross-entropy loss, $\lambda$ is the weight decay hyper-parameter, $N_i$ is the number of samples for client i and $\sum_{i=1}^K N_i = N$.
            \STATE \textbf{Server runs:}
            \begin{ALC@g}
            \FOR{each round $t = 0, 1, 2, ..., T-1$}
            \IF[Supervised Round]{$(T \bmod{2A}) < A$ }  
                \FOR{each supervised client $s$ \textbf{in parallel}}
                    \STATE $\theta_{t+1}^{s}  \leftarrow \text{SupervisedTraining}(s, \theta_t)$
                \ENDFOR
                \STATE $\theta_{t+1} \leftarrow \sum_{s=1}^{S} \frac{N_{s}}{N} \theta_{t+1}^{s}$
            \ELSE[Unsupervised Round]
                \FOR{each unsupervised client $u$ \textbf{in parallel}}
                    \STATE $\theta_{t+1}^{u}  \leftarrow \text{UnsupervisedTraining}(u, \theta_t)$
                \ENDFOR
                \STATE $\theta_{t+1} \leftarrow \sum_{u=S+1}^{K} \frac{N_{u}}{N} \theta_{t+1}^{u}$
            
            \ENDIF
     
            \ENDFOR
            \end{ALC@g}
            \STATE 
            \STATE \textbf{SupervisedTraining}($s$, $\theta$): // \textit{Supervised client $s$}
            \begin{ALC@g}
            \FOR{$e$ in epoch}
            \FOR{minibatch $x$ in training data}
            \STATE $p = f_{\theta}(x)$
            \STATE $\mmL_{\mathrm{tr}}(\theta) = DL(p, y) + CE(p, y)$
            \STATE Update $\theta = \theta - \gamma_\theta \nabla_\theta\mmL_{\mathrm{tr}}(\theta)$
            % \STATE Update 
            % \STATE $\alpha = \alpha - \eta_\alpha \left(\nabla_\alpha  \mmL_{\mathrm{tr}}(w, \alpha) +  \lambda \nabla_\alpha \mmL_{\mathrm{val}} (w, \alpha)\right)$
            \ENDFOR
            \ENDFOR
            \STATE return $\theta$ to server
            \end{ALC@g}
            \STATE 
            \STATE \textbf{UnsupervisedTraining}($u$, $\theta$): // \textit{Unsupervised client $u$}
            \begin{ALC@g}
            \STATE $\xi \leftarrow \theta$ // \textit{initialize student model parameters with the global model parameters}
            \FOR{$e$ in epoch}
            \FOR{sample two batches ($x_1$, $x_2$) in training data}
            \STATE $x^{'} = Mixup(x_1, x_2)$
            \STATE $p_{mix} = f_{\xi}(x_{mix})$
            \STATE $p_{1} = f_{\theta}(x_1)$, $\quad$ $p_{2} = f_{\theta}(x_2)$
            \STATE $p^{'} = Mixup(p_{1}, p_{2})$
            \STATE $y = argmax(p^{'})$
            \STATE $\mmL_{\mathrm{tr}}(\xi) = DL(p_{mix}, y) + CE(p_{mix}, y)$
            
            \STATE Update $\xi = \xi - \gamma_\xi 
            \nabla_\xi\mmL_{\mathrm{tr}}(\xi)$
            \STATE Update $\theta = \tau \theta + (1 - \tau ) \xi$
            % \STATE Update 
            % \STATE $\alpha = \alpha - \eta_\alpha \left(\nabla_\alpha  \mmL_{\mathrm{tr}}(w, \alpha) +  \lambda \nabla_\alpha \mmL_{\mathrm{val}} (w, \alpha)\right)$
            \ENDFOR
            \ENDFOR
            \STATE return $\theta$ to server
            \end{ALC@g}
        \end{algorithmic}
    \end{small}
\label{alg:fssl}
\end{algorithm}

